Saturn Platform: Foundation Model Operations and Generative AI for Financial Services

Saturn is an innovative platform that assists Foundation Model (FM) building and its integration with IT operations (Ops). It is custom-made to meet the requirements of data scientists, enabling them to effectively create and implement FMs while enhancing collaboration within their technical domain. By offering a wide range of tools and features, Saturn streamlines and automates different stages of FM development, making it an invaluable asset for data science teams. This white paper introduces prospective applications of generative AI models derived from FMs in the financial sector.

==> imgs/name.tex <==
Espero que esta avaliação seja considerada construtiva.

Durante este ano, observei o Marcos rejeitar projetos cruciais para nossa área sem uma justificativa clara. Exemplos notáveis incluem o Modelo Fundacional Financeiro e a Plataforma Saturn, nos quais não apenas negou apoio, mas desencorajou sua implementação. Apesar da oposição, minha equipe perseverou e desenvolveu esses projetos discretamente. Surpreendentemente, Marcos agora atribui esses projetos a iniciativas institucionais, sugerindo alinhamento, enquanto, na realidade, sua oposição foi uma barreira prejudicial para minha equipe.

A intervenção direta de Marcos no projeto Personas causou um desgaste desnecessário em minha equipe. Acredito que o papel de um diretor-executivo não deve incluir microgerenciamento de equipes de ciência de dados. A falta de conhecimento de Marcos sobre métodos contemporâneos de ciência de dados e suas imposições não validadas comprometeram a qualidade do modelo, além de impedir a colaboração com os times de negócios e potenciais usuários. Essa interferência prejudicou a adoção do modelo no banco.

A falta de ação do Marcos para resolver conflitos internos resultou em redundâncias desnecessárias, com equipes desenvolvendo tecnologias similares às já existentes, porém notavelmente inferiores, comprometendo os avanços significativos alcançados pela minha equipe em MLOps e produtização de modelos.




































